HybridSim: A Physics-Learning Hybrid Digital Twin for mmWave Human Sensing

High-fidelity simulation of mmWave radar signals for dynamic human motion is valuable for developing radar-based human sensing models; yet collecting accurately labeled measurements for a specific deployment site remains expensive. We present HybridSim, a physics-learning hybrid simulator that synthesizes mmWave radar signals from dynamic human meshes under a fixed indoor room configuration, explicitly decoupling propagation into two components. To parameterize the human subject, we use a tri-plane representation to extract human features and a Graph Convolutional Network to stabilize optimization and mitigate gradient instability. The direct signal path is modeled via an inverse-rendering formulation with a microfacet BRDF to capture primary surface reflections. In parallel, the indirect path is approximated by combining 3D Gaussian Splatting with a virtual-receiver geometry to fit and reproduce site-specific multipath interference patterns, achieving substantially lower computational cost than explicit full ray tracing. Experiments in a fixed-room setting show improved agreement with a physically based reference and consistent gains on downstream radar-based human sensing tasks when using HybridSim for site-specific data augmentation.

==> table/pose_est.tex <==
% \begin{table}[t]
% \centering
% \caption{test on evaluation set (action 9-24)}
% \label{tab:pose_est}
% \begin{tabular}{lcccc}
% \toprule
% Methods & Q($^\circ$) & S(cm) & V(cm) & T(cm) \\
% \midrule
% mmGPE   & 16.44 & 9.11 & 11.52 & 5.00\\mean = (16.435197, 0.050046, 0.115191, 0.091053, 1.000000)
% Ours    & 14.57 &  & 7.95 & 9.98 & 4.42 \\ %train 48000
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{test on training set (action 1-8)}
% \label{tab:pose_est}
% \begin{tabular}{lcccc}
% \toprule
% Methods & Q($^\circ$) & S(cm) & V(cm) & T(cm) \\
% \midrule
% mmGPE   &  &  &  & \\mean = (11.300870, 0.031460, 0.086674, 0.069174, 0.999999)
% Ours    & 9.02 &  & 6.59 & 7.74 & 4.38 \\ %train 6000 mean(angle, trans, vert, ske, betas) = (9.016442, 0.043808, 0.077437, 0.065901, 0.999999)
% \bottomrule
% \end{tabular}
% \end{table}
\begin{table}[t]
\centering
\caption{Pose Estimation Results on Training Set (Action 1-8) and Evaluation Set (Action 9-24)}
\label{tab:pose_est}
\begin{tabular}{llcccc}
\toprule
Dataset & Methods & Q($^\circ$) & S(cm) & V(cm) & T(cm) \\
\midrule
\multirow{2}{*}{Training Set (Action 1-8)}
    & mmGPE & 11.30 & 6.92 & 8.67 & 3.15 \\
    & Ours  & 9.02 & 6.59 & 7.74 & 4.38 \\
    & Ours (w. MVDR) & 8.88 & 5.62 & 6.80 & 3.28\\ %24000: 8.884360  0.032818  0.068025  0.056217
\midrule
\multirow{2}{*}{Evaluation Set (Action 9-24)}
    & mmGPE   & 16.44 & 9.11 & 11.52 & 5.00\\
    & Ours    & 14.57 & 7.95 & 9.98 & 4.42 \\ %train 48000
    & Ours (w. MVDR)   & 14.22 & 7.83 & 9.90 & 3.95\\ %38000
\bottomrule
\end{tabular}
\end{table}

